Structured Variational Inference in Continuous Cox Process Models

We propose a scalable framework for inference in an inhomogeneous Poisson process modeled by a continuous sigmoidal Cox process that assumes the corresponding intensity function is given by a Gaussian process (GP) prior transformed with a scaled logistic sigmoid function. We present a tractable representation of the likelihood through augmentation with a superposition of Poisson processes. This view enables a structured variational approximation capturing dependencies across variables in the model. Our framework avoids discretization of the domain, does not require accurate numerical integration over the input space and is not limited to GPs with squared exponential kernels. We evaluate our approach on synthetic and real-world data showing that its benefits are particularly pronounced on multivariate input settings where it overcomes the limitations of mean-field methods and sampling schemes. We provide the state of-the-art in terms of speed, accuracy and uncertainty quantification trade-offs.

==> figure_taxi.tex <==
\begin{center}
	\begin{figure}[h]
		\includegraphics[width=1.0\textwidth,height=\textheight,keepaspectratio]{images/real/taxi_dataset_D_O_L}
		\caption{Predictive mean intensity.}
	\end{figure}
	\label{fig:synthetic}
\end{center}

==> real_taxi.tex <==
\begin{center}
	\begin{figure}[h]
		\includegraphics[width=0.9\textwidth,height=\textheight,keepaspectratio]{images/real/taxi_dataset_D_O}
		\caption{1 realisations for each function}
	\end{figure}
	\label{fig:synthetic}
\end{center}

==> references.tex <==
\bibliographystyle{apalike}
\bibliography{references}


==> table_related_work.tex <==

\begin{table}[]
\begin{minipage}[t]{0.4\textwidth}
\begin{tabular}{lllll}
\textit{}       & \multicolumn{1}{c}{\textbf{Inference}} & \textbf{Link function} & \textbf{Input space} &  \\
\our             & \textit{}                              & \textit{}              & \textit{}            &  \\
\donner          & \textit{}                              & \textit{}              & \textit{}            &  \\
\lloyds & \textit{}                              & \textit{}              & \textit{}            &  \\
\lgcp            &                                        &                        &                      &  \\
gunter          &                                        &                        &                      &  \\
lian            &                                        &                        &                      & 
\end{tabular}
\end{minipage}
\end{table}


==> table_taxi.tex <==

Taxi data:
\begin{tabular}{lrrr}
	\hline
	Method   &    NLPL &   Test log lik &   Time(s) \\
	\hline
	OUR      & -379936 &        -386404 &    121.71 \\
	Donner   & -595491 &        -601972 &      0.42 \\
	\hline
\end{tabular}
